Mixed H2/H-infinity Data-Driven Control Design for Hard Disk Drives

A frequency based data-driven control design considering mixed H2/H-infinity control objectives is developed for multiple input-single output systems. The main advantage of the data-driven control over the model-based control is its ability to use the frequency response measurements of the controlled plant directly without the need to identify a model for the plant. In the proposed methodology, multiple sets of measurements can be considered in the design process to accommodate variations in the system dynamics. The controller is obtained by translating the mixed H2/H-infinity control objectives into a convex optimization problem. The H-infinity norm is used to shape closed loop transfer functions and guarantee closed loop stability, while the H2 norm is used to constrain and/or minimize the variance of signals in the time domain. The proposed data-driven design methodology is used to design a track following controller for a dual-stage HDD. The sensitivity decoupling structure[16] is considered as the controller structure. The compensators inside this controller structure are designed and compared by decoupling the system into two single input-single-output systems as well as solving for a single input-double output controller.

==> 4-Example/4-ApplicationDD-DesignResult.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Control Design Settings}
%%%%%%%%%%%%%%%%%%%%%%%%
%%% plants
In this section, the data driven mixed $H_2/H_\infty$ control design methodology will be used to design a track following controller for a dual-stage HDD. As previously stated, the data-driven design methodology only uses frequency response measurements of the plant, without requiring models of the actuators. Here, five sets of frequency response data are used to represent dynamics variations for each actuator. These five frequency response data are plotted in Fig. \ref{fig:SISO:G}. If a higher number of frequency response data is required to represent system dynamics, those measurements can be easily included in the design process. The frequency response plots shown in Fig.~\ref{fig:SISO:G} were generated using realistic models of both the VCM and the MA. The data-driven design methodology presented in this dissertation was also used with real frequency response data provided by our HDD industrial research partners. However, this data is considered confidential and proprietary by our partners and cannot be presented here. Therefore, the frequency response data plotted in Fig.~\ref{fig:SISO:G} were produced to mimic real measurements.
\begin{figure}
	\centering
	\includegraphics[width=8cm]{Pictures/5mdl_G.jpg}
	\caption{Hard disk drive actuators frequency response measurements used in the design. Five measurements from each actuator is used in the design. $G_v$ and $G_m$ represent VCM and MA actuators' transfer functions, respectively. The actuators output units for both the VCM and the MA are 10 nm.}
	\label{fig:SISO:G}
\end{figure}
%It is worth mentioning that the track following controller for a dual-stage HDD is designed using the realistic measurements of HDD actuators provided by our HDD industry partners. However, those measurements are HDD industry confidential data and cannot be shown here.

%%% noises
%There are four sources of external noises and disturbances considered to be applied on the hard disk drives as shown in Fig. \ref{fig:AppDD:DualSD}. $n$ is contaminating the measurement signal and is called the measurement noise. $w_v$ and $w_m$ are the control input noises and the $r$ is the run-out. The major sources for these noises and disturbances are the windage caused by the rotation of the magnetic disk, external vibrations and also the measurement noises. 
%The closed loop transfer functions from run-out $r$ and control input noises $w_v,~w_m$ to control inputs and noises have been considered as $H_\infty$ constraints to shape the closed loop transfer functions. However, the 

\subsubsection{Noise Spectrum}
The noise spectrum considered for the $H_2$ norm computations in Eqs.~(\ref{eq:H2:E:dual})-(\ref{eq:H2:mY:dual}) are shown in Fig.~\ref{fig:SISO:noises} for the run-out $R$ and measurement noise $N$. The spectrum are denoted with the upper-case letters of the corresponding noises. These spectrum data will be used directly in the design process without any model fitting. According to our HDD industrial research partners, the spectrum for the control input noises can be set to zero, $W_v=0$ and $W_m=0$, since the spectrum given in Fig.~\ref{fig:SISO:noises} are obtained by assuming that the effects of control input noises are lumped into the run-out $R$ and measurement noise $N$ spectrum. Although the spectrum for the control input noises are set to zero, the closed loop transfer functions from control input noises to control inputs and error signals are considered in the design as $H_\infty$ constraints.

%In the examples presented in this section, it is assumed that the effects of control input noises in Figs.~\ref{fig:AppDD:DualSD} and \ref{fig:AppDD:Single} are lumped into the run-out $r$ and measurement noise $n$. Fig. \ref{fig:SISO:noises} shows the frequency response data of the spectrum for these two noises. The spectrum are denoted with the upper-case letters of the corresponding noises. These spectrum data will be used directly in the design process without any model fitting.% any model to these spectrum.
\begin{figure}
	\centering
	\includegraphics[width=8cm]{Pictures/mdl_noises2.jpg}
	\caption{Estimated spectrum of external noises applied on the hard disk drive. $R$ and $N$ respectively represent the spectrum for the run-out $r$ and the measurement noise $n$.}
	\label{fig:SISO:noises}
\end{figure}

\subsubsection{$H_\infty$ Constraints}
%%% constraints: Hinf
The $H_\infty$ constraints used in the optimization problems are weighted using numerically shaped bounded weighting functions over the frequency regions. As mentioned in section~\ref{sec:DD:ControlObjective}, the SISO transfer functions are shaped using the inverse of these weighting functions. Moreover, the maximum singular values of the MIMO transfer functions are shaped using the inverse of the minimum singular values of these weighting functions. These shaping functions are shown with light blue dotted lines in Appendix~\ref{ch:Appendix:HinfResults} and are called the $H_\infty$ constraint limits. The scalar $\gamma$ used in all $H_\infty$ constraints is chosen to be $1$. 

\subsubsection{$H_2$ Constraints}
%%% constraints: H2
The $H_2$ constraints in Eqs.~(\ref{eq:H2:vU:single}), (\ref{eq:H2:vU:dual}) and (\ref{eq:H2:mY:dual}) are used to constraint the variances of the VCM input and the MA output stroke in time domain. Since the standard deviation is the square root of the variance, the upper-limits for the standard deviations of the VCM control input both in the VCM single-stage and dual-stage loops are chosen to be
\begin{equation}\label{eq:dual:H2:vUnumbers}
\eta_{u_v^s}=2.0~v,~\eta_{u_v}=2.0~v,
\end{equation}
respectively. Four different values for the standard deviation upper-limit of the MA output stroke will be considered:
\begin{equation}\label{eq:dual:H2:mYnumbers}
\eta_{y_m}=44,~42,~40,~38~nm.
\end{equation}
By varying the standard deviation upper-limit of the MA output stroke in Eq.~(\ref{eq:H2:mY:dual}), we can study the effect of restraining the MA's stroke on the overall HDD track following servo performance.

\subsubsection{Controller Structure}
%%% Ghm, z/z-1
The sensitivity decoupling controller structure given in Fig.~\ref{fig:AppDD:DualSD} is used for the dual-stage HDD control design. The estimated model of the MA plant used in the controller structure is considered to be a pure delay
\begin{equation}
\hat{G}_m = \frac{1}{z}.
\end{equation}
Moreover, an integrator of the form $\frac{z}{1-z}$ is incorporated into the VCM controller, in order to eliminate the steady state tracking error due to the DC disturbances. As mentioned in Section~\ref{sec:AppDD:Structure}, the compensators $K_v$ and $K_m$ can be obtained using either the sequential SISO or SIMO design strategies. In the sequential SISO design strategy, these compensators are obtained in two consecutive steps, while in the SIMO design strategy, $K_v$ and $K_m$ are obtained simultaneously. 

\subsubsection{Stable Factorizations}
%%% factorizations: simo
The stable factorizations of a SIMO controller with an integrator included in the first element of the controller was derived in Eqs.~(\ref{eq:MISO:fact:Xi}) and (\ref{eq:MISO:fact:Yi}). In these equations, the value of the parameter $m$ is $2$, since the SIMO controller for the dual-stage HDD has two outputs. Moreover, the controller order parameter, $n$, is selected to be $25$.

%%% factorizations: siso
In the sequential SISO design strategy, first the compensator $K_v$ is obtained using the VCM single-stage loop in Fig.~\ref{fig:AppDD:Single}. Then, the compensator $K_m$ is obtained using the dual-stage loop in Fig.~\ref{fig:AppDD:DualSD} given the obtained compensator $K_v$. The first SISO design step for obtaining the compensator $K_v$ uses the controller stable factorizations in Eqs.(\ref{eq:MISO:fact:Xi}) and (\ref{eq:MISO:fact:Yi}), which consider an integrator in the controller structure. Since this is a SISO loop, $m=1$ is chosen. The compensator $K_m$ uses stable factorizations given in Eqs.~(\ref{eq:MISO:fact:X}) and (\ref{eq:MISO:fact:Y}) with $m=1$. The compensator order parameter, $n$, for $K_v$ and $K_m$ is chosen to be $16$ and $20$, respectively. It will be shown later in this section, that the compensator order reduction for the SIMO design strategy with $n=25$ will lead to the mentioned compensator orders in the sequential SISO design strategy.

%%% parameterizations: G
The actuators in the HDD are stable actuators. Therefore, the initial stable factorizations of the actuators frequency response measurements are obtained using Eqs. (\ref{eq:MISO:Factorization:Gstable:N}) and (\ref{eq:MISO:Factorization:Gstable:M}). As mentioned in the mixed $H_2/H_\infty$ flowchart in Fig.~\ref{fig:SISO:MixedH2Hinf}, these stable factorizations are normalized at the end of each iteration using Eq. (\ref{eq:MN:normalize}).

\subsubsection{Design Scenarios}
%%% Forming convex optimization problems
Once the stable factorizations for the actuators and controllers are defined, the convex optimization problems mentioned in Section~\ref{sec:AppDD:Algorithm} are formulated and solved. The sequential SISO controller design strategy solves the optimization problems formulated in Eqs. (\ref{eq:opt:sd:single:II}) and (\ref{eq:opt:sd:dual:II}) for the compensators $K_v$ and $K_m$, respectively. The SIMO controller is obtained by solving Eq. (\ref{eq:opt:miso:II}). %The $H_\infty$ constraints mentioned in these equations have been weighted using numerically shaped weighting functions over the frequency regions. The inverse of these weighting functions have been shown with dotted lines in Appendix~\ref{ch:Appendix:HinfResults}. 

% %%% constraints: Hinf, H2
% The $H_\infty$ constraints used in the optimization problems are weighted using numerically shaped bounded weighting functions over the frequency regions. As mentioned in section~\ref{sec:DD:ControlObjective}, the SISO transfer functions are shaped using the inverse of these weighting functions. Moreover, the maximum singular values of the MIMO transfer functions are shaped using the inverse of the minimum singular values of these weighting functions. These shaping functions are shown with light blue dotted lines in Appendix~\ref{ch:Appendix:HinfResults} and are called the $H_\infty$ constraint limits. The scalar $\gamma$ used in all $H_\infty$ constraints is chosen to be $1$. 



% %The inverse of these weighting functions for the SISO transfer functions and the inverse of the minimum singular values of these weighting functions for the MIMO transfer functions are shown with light blue dotted lines in Appendix~\ref{ch:Appendix:HinfResults}. 

% %The $H_\infty$ constraints used in the optimization problems are weighted using numerically shaped bounded weighting functions over the frequency regions. The inverse of these weighting functions are shown with light blue dotted lines in Appendix~\ref{ch:Appendix:HinfResults}. Also, the scalar $\gamma$ used in the $H_\infty$ constraints is chosen to be $1$. 

% The $H_2$ constraints in Eqs.~(\ref{eq:H2:vU:single}), (\ref{eq:H2:vU:dual}) and (\ref{eq:H2:mY:dual}) are used to constraint the variances of the VCM input and the MA output in time domain. The upper-limits for the $H_2$ norms of the VCM control input both in the VCM single-stage and dual-stage loops have chosen to be
% \begin{equation}\label{eq:dual:H2:vUnumbers}
% \eta_{u_v^s}=2.0,~\eta_{u_v}=2.0,
% \end{equation}
% respectively. Four different values for the $H_2$ norm upper-limit of the MA output will be considered:
% \begin{equation}\label{eq:dual:H2:mYnumbers}
% \eta_{y_m}=4.4,~4.2,~4.0,~3.8
% \end{equation}
% in both the sequential SISO and the SIMO design strategies. By varying the $H_2$ norm upper-limit of the MA output variance in Eq.~(\ref{eq:H2:mY:dual}), we can study the effect of restraining the MA's stroke on the overall HDD track following servo performance.


%%% design scenarios
%The controllers in the sensitivity decoupling structure given in Fig.\ref{fig:AppDD:DualSD} have been designed using both SISO and SIMO methodologies. 
The compensators in the sensitivity decoupling structure given in Fig.~\ref{fig:AppDD:DualSD} are designed and compared under different scenarios for the standard deviation upper-limit of the MA output stroke and design strategies. The compensators obtained using the sequential SISO design strategy always satisfied all the four constraints for the standard deviation of the MA output stroke. Therefore for the sake of simplicity, only the $\eta_{y_m}=44$ scenario is considered for the sequential SISO design strategy. Table~\ref{table:design:scenarios} presents the five cases of controller design scenarios compared in this section as well as their respective color code used in the plots.
% \begin{table}[ht]
% \caption{Controller design scenarios and their color code.} % title of Table
% \centering % used for centering table
% \begin{tabular}{c c c c c c} % centered columns (4 columns)
% \hline\hline %inserts double horizontal lines
% Scenarios 				& 	$SIMO_1$	&	$SIMO_2$ 	& $SIMO_3$ 		& 	$SIMO_4$ 	& 	$SISO_1$\\ [0.5ex] 
% 		 			    %&	$dB$		& 	$dB$ 	& $degree$ 	& 	$Hz$ 			& 	$Hz$ \\ [0.5ex]
% \hline 
% \text{Design strategies}  &	SIMO	&	SIMO 	& SIMO 		& 	SIMO 	& 	sequential SISO    \\
% \text{$\eta_{y_m}$ (nm)}  &	44  & 42  &  40 	 & 	38 			& 	44    \\
% \text{Color code}  &	\textcolor{blue}{\rule{1cm}{1mm}}  & \textcolor{magenta}{\rule{1cm}{1mm}}   &  \textcolor{green}{\rule{1cm}{1mm}} 	 &  \textcolor{red}{\rule{1cm}{1mm}}			& 	\textcolor{black}{\rule{1cm}{1mm}}    \\ [1ex] % [1ex] adds vertical space
% \hline %inserts single line
% \end{tabular}
% \label{table:design:scenarios} % is used to refer this table in the text
% \end{table}


\begin{table}[ht]
\caption{Controller design scenarios and their color code.} % title of Table
\centering % used for centering table
\begin{tabular}{c c c c } % centered columns (4 columns)
\hline\hline\\[-0.8em] %inserts double horizontal lines
\text{Scenarios} 				& 	\text{Design strategies}	&	\text{$\eta_{y_m}$ (nm)} 	& \text{Color code}		\\ [0.5ex] 
		 			    %&	$dB$		& 	$dB$ 	& $degree$ 	& 	$Hz$ 			& 	$Hz$ \\ [0.5ex]
\hline \\[-0.5em]
$SIMO_1$  &	SIMO	&	44 	& \textcolor{blue}{\rule{1cm}{1mm}} \\ [1ex]
$SIMO_2$  &	SIMO	&	42 	& \textcolor{magenta}{\rule{1cm}{1mm}} \\ [1ex]
$SIMO_3$  &	SIMO	&	40 	& \textcolor{green}{\rule{1cm}{1mm}} \\ [1ex]
$SIMO_4$  &	SIMO	&	38 	& \textcolor{red}{\rule{1cm}{1mm}} \\ [1ex]
$SISO_1$  &	Sequential SISO	&	44 	& \textcolor{black}{\rule{1cm}{1mm}} \\ [1ex] % [1ex] adds vertical space
\hline %inserts single line
\end{tabular}
\label{table:design:scenarios} % is used to refer this table in the text
\end{table}

%%% design: 10 iterations => H2 kicks in
The design approach proposed in chapter~\ref{ch:DataDriven} is an iterative approach. Here, the controllers are designed using $10$ iterations. As shown in the flowchart given in Fig.~\ref{fig:SISO:MixedH2Hinf}, the first iteration only considers the $H_\infty$ constraints. The second iteration will include the $H_2$ objective. Finally starting from the third iteration, the full optimization problem including $H_2$ objective, $H_2$ and $H_\infty$ constraints will be considered. 

%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Design Results}
%%%%%%%%%%%%%%%%%%%%%%%%
%%% Results: Hinf constraints
In this section, the controllers are designed for the dual-stage HDD considering the design scenarios mentioned in the previous section. The design criteria for both the VCM single-stage and the dual-stage loops are included in the design process. First, the controller design results for both of these loops are discussed considering all the design scenarios in Table~\ref{table:design:scenarios}. Then,  an example to describe the limitation of the sequential SISO design strategy compared to the SIMO design strategy is provided. Last but not the least, the sufficient condition for the $H_\infty$ criteria mentioned in theorem~\ref{theorem:miso:Hinf:Karimi} and the necessary and sufficient condition mentioned in theorem~\ref{THEOREMMISOHINF} are compared in an example of the data-driven mixed $H_2/H_\infty$ control design.

\subsubsection{Design Scenarios Comparison}
The closed loop transfer functions in the final iteration, $10^{th}$ iteration, and their $H_\infty$ constraint limits for VCM single-stage and dual-stage loops are shown in Appendix~\ref{ch:Appendix:HinfResults}. As one can observe, all the closed loop transfer functions satisfy the $H_\infty$ constraints given in Eqs.~(\ref{eq:Hinf:single}), (\ref{eq:Hinf:dual:overall}), (\ref{eq:Hinf:dual:individual:E}) and (\ref{eq:Hinf:dual:individual:U}). One of the main advantages of the data-driven approach over the model-based approaches is that the weighting functions used to shape the closed loop transfer functions can be numerically shaped.


%%% Results: single loop
The $H_2$ norm objective and constraints, for the VCM single-stage loop depicted in Fig.~\ref{fig:AppDD:Single} are shown in Fig.~\ref{fig:single:H2}, considering all the scenarios mentioned in table~\ref{table:design:scenarios}. According to the SISO optimization problem for the VCM single-stage loop given in Eq. (\ref{eq:opt:sd:single:II}), the objective is to minimize the variance of the VCM single-stage tracking error while designing the VCM controller. However, the objective in the MISO design strategy is to minimize the variance of the dual-stage tracking error, without considering the variance of the single-stage tracking error as an optimization objective. Therefore, as one can notice in Fig.~\ref{fig:single:H2:S}, the sequential SISO design strategy achieves the smallest square root of the variance, standard deviation, for the VCM single-stage tracking error as compared to the SIMO designs. Moreover, Fig.~\ref{fig:single:H2:vU} shows that the controller designed using the sequential SISO strategy has the highest activity in terms of the control input standard deviation.

%the MISO design strategy only considers the $H_2$ norm of the dual-stage tracking error as the minimization objective. Therefore, as one can observe in Fig.~\ref{fig:single:H2:S}, the sequential SISO design strategy achieves the smallest $H_2$ norm for the VCM single-stage tracking error compared to the SIMO designs. Moreover, Fig.~\ref{fig:single:H2:vU} shows that the controller designed using the sequential SISO strategy has the highest activity in terms of $H_2$ norm of the control input.% uses the maximum allowed $H_2$ norm of the control input to minimize the single-stage tracking error.
\begin{figure}
    \centering
    \begin{subfigure}[b]{8cm}
        \includegraphics[width=8cm]{Pictures/5mdl_single_H2_S_2.jpg}
        \caption{$\norm{e^s}_2$}
        \label{fig:single:H2:S}
    \end{subfigure}
    \begin{subfigure}[b]{8cm}
        \includegraphics[width=8cm]{Pictures/5mdl_single_H2_vU.jpg}
        \caption{$\norm{u^s_v}_2$}
        \label{fig:single:H2:vU}
    \end{subfigure}
    \caption{The $H_2$ norm objective and constraints, for the VCM single-stage loop depicted in Fig.~\ref{fig:AppDD:Single} over the iterations. The variances of signals is considered in the optimization problems, however the square roots of the variances, also known as the standard deviations, are plotted here. The triangles show the upper-bound of the standard deviations of the tracking error (a) and the VCM control action (b), where the circles show the real values of the standard deviations. The $H_2$ norm objective and constraints are activated starting from the second and third iterations, respectively.}\label{fig:single:H2}
\end{figure}

%%% single: effect of MA restriction
%In the SIMO design methodology, the objective is to minimize the dual-stage tracking error. 
The MA output stroke is restricted by defining an upper-bound on its variance in Eq.~(\ref{eq:H2:mY:dual}). Reducing the value of this upper-bound will create more restriction on the MA output stroke. The more restriction on the MA output stroke will reduce the MA ability to minimize the tracking error. In this case, the sensitivity decoupling structure suggests that the VCM should compensate for the MA by achieving a smaller standard deviation of the VCM single-stage tracking error. As shown in Figs.~\ref{fig:single:H2:S} and \ref{fig:single:H2:vU}, the VCM single-stage loop will achieve smaller tracking error standard deviations at the cost of having increased VCM control input standard deviations, if there is more restriction on the MA output stroke.

%%% single: Table, Sr explanation
As shown in Fig.~\ref{fig:single:H2:S}, the controller designed using the sequential SISO design strategy is the most aggressive one in terms of minimizing the standard deviation of the VCM single-stage tracking error. Also, the SIMO controllers with more restriction on the MA output stroke will be more aggressive based on this definition. The VCM single-stage sensitivity plots for all these scenarios are shown in Fig.~\ref{fig:single:Er}. In the frequency region between $0-500~Hz$ where the VCM is the dominant actuator, all these scenarios achieve almost the same level of VCM single-stage tracking error reduction. However in the frequency region between $500-2000~Hz$ where both actuators are active, the more aggressive VCM single-stage controller will improve the VCM single-stage tracking error reduction, in order to compensate for the MA output stroke restriction. 

Table~\ref{table:single:Margins} shows the stability margins and bandwidths for all these controllers. The more aggressive controller generally pushes the bandwidth, $\omega_{PM}$, at the cost of having lower stability margins. However, this trend is not completely followed, since the aggressiveness of the controllers is defined in terms of the $H_2$ norm of the closed loop transfer functions, which restricts the integration of the frequency response magnitude over the entire frequency region. Therefore, increasing the restriction on the $H_2$ norm will not always directly affect the bandwidth and stability margins.%can lead to smaller $H_2$ norm but it may create sharp peaks at few frequency regions, which can compromise stability margin.

%The $H_2$ norm constraints restrict the integration of the frequency response magnitude over the whole frequency region. Therefore, increasing the restriction on $H_2$ norm can lead to smaller $H_2$ norm but it can create sharp peaks at few frequency regions. As one can see in Fig.~\ref{fig:dual:H2cst:mY}, increasing the restriction on MA output, have reduced the $H_2$ norm of the MA output, but it has increased the magnitude of the pick in the frequency response plot of MA output in Fig.~\ref{fig:dual:Tr}. If the $H_2$ norm constraints create the peaks which reduce the stability margins or violate performance specifications, those peaks will be bounded by shaping the closed loop transfer functions using the weighted $H_\infty$ constraints.


%The single-stage sensitivity plots for all these scenarios have been shown in Fig.~\ref{fig:single:Er}. In $1000-2000~Hz$ frequency region where both actuators are active, the more aggressive controller has been more successful in terms of error reduction. This improved error reduction will help the dual-stage error reduction for the more restricted MA. Table~\ref{table:single:Margins} shows the stability margins and bandwidths for all these controllers. The general trend for the single-stage loop is that the more aggresive controller will achieve higher  single-stage bandwidth, $\omega_{PM}$ , at the cost of having lower stability margins. However, this trend has not been completely followed, since it is not explicitly considered in the design.

%all these scenarios achieve almost the same level of error reduction below $500-600~Hz$. However in the frequency region $500-2000~Hz$, where the MA start , however in the middle frequency regio, where a more aggressive controller will increase the peak magnitude of this transfer function.

%Table~\ref{table:single:Margins} shows the stability margins and bandwidths for all these controllers. As one can see, the more aggressive controller will achieve higher single-stage bandwidth, $\omega_{PM}$. However, the stability margins are not following a unique trend, since  .....%%%, at the cost of having lower stability margins. The reduction in stability margins can be observed as the significant reduction in gain margin and increase in the peak magnitude of the sensitivity plot. The single-stage sensitivity plot is also shown in Fig.~\ref{fig:single:Er}, where a more aggressive controller will increase the peak magnitude of this transfer function.%%%
\begin{table}[ht]
\caption{Stability margins for the VCM single-stage loop} % title of Table
\centering % used for centering table
\begin{tabular}{c c c c c c} % centered columns (4 columns)
\hline\hline\\[-0.8em] %inserts double horizontal lines
Scenarios 				& 	$E^s_{r \rightarrow e}$ peak	&	$GM$ 	& $PM$ 		& 	$\omega_{GM}$ 	& 	$\omega_{PM}$\\ [0.5ex] 
		 			    &	$dB$		& 	$dB$ 	& $degree$ 	& 	$Hz$ 			& 	$Hz$ \\ [0.5ex]
\hline \\[-0.5em]
\text{$SIMO_1$}  &	9.97  & 3.45  &  25.83 	 	& 	2,206 			& 	1,242    \\
\text{$SIMO_2$}  &	10.01  & 3.30  &  28.55 	 	& 	2,319			& 	1,230    \\
\text{$SIMO_3$}  &	10.17  & 3.22  &  31.17 	 	& 	2,427			& 	1,244    \\
\text{$SIMO_4$}  &	10.03 & 3.28   &  32.46	 		& 	2,548			& 	1,276    \\
\text{$SISO_1$}   & 10.10 & 3.28   &  31.45 	 	& 	2,493			&	1,344    \\ [1ex] % [1ex] adds vertical space
\hline %inserts single line
\end{tabular}
\label{table:single:Margins} % is used to refer this table in the text
\end{table}

\begin{figure}
	\centering
	\includegraphics[width=8cm]{Pictures/5mdl_single_Sr.jpg}
	\caption{The magnitude Bode plots of VCM single-stage sensitivity transfer function, $E^s_{r \rightarrow e}$.}
	\label{fig:single:Er}
\end{figure}
%The single-stage closed loop transfer function from the run-out, $r$, to the tracking error, $e$, has been given in Fig.~\ref{fig:single:Er}. As mentioned, the SISO design will result in the most aggressive VCM controller, and in the SIMO design, restricting the MA output will make the VCM controller more aggressive. As one can see in Table~\ref{table:single:Margins} and Fig.~\ref{fig:single:Er}, having a more aggressive controller, will increase bandwidth at the cost of reduction in the stability margin.


% Dual-stage mY, vU for SISO
% Dual-stage S: SD higher than MISO => mY

% Dual: siso vs miso: bw & stability margin
% Dual: among miso
% Dual: Tr

%%% Results: Dual-stage 
The $H_2$ norm constraints for the VCM input and the MA output stroke in the dual-stage HDD are shown in Figs.~\ref{fig:dual:H2cst:vU} and~\ref{fig:dual:H2cst:mY}, respectively. In the sequential SISO design strategy, the VCM is designed to be aggressive. As a result, the standard deviation of the VCM input in both the VCM single-stage and dual-stage settings for the sequential SISO design strategy will be higher compared to all the scenarios in the SIMO design strategy, according to Figs.~\ref{fig:single:H2:vU} and \ref{fig:dual:H2cst:vU}. As mentioned in the SIMO design strategy, the more restriction on the MA output stroke has the effect of increasing the standard deviation of the VCM control input in the VCM single-stage setting to compensate for the MA output stroke restriction. However, this restriction will decrease the standard deviation of the VCM control input in the dual-stage setting, since this restriction requires less VCM movements to compensate for the MA output movements which are out of phase with the VCM output movements. Fig.~\ref{fig:dual:H2cst:mY} demonstrates that all the controller design scenarios considered in table~\ref{table:design:scenarios} are satisfying their standard deviation upper-bound constraints for the MA output stroke.%Moreover, the SIMO design methodlogy will achieve smaller $H_2$ norm for the VCM control input, if the MA output has more restriction. This trend ...



%the VCM is the single-stage setting has already been helpful in reducing the tracking error, and the restriction in dual-stage wi
%my: movements => in phase with vcm input => 

\begin{figure}
    \centering
    \begin{subfigure}[b]{8cm}
        \includegraphics[width=8cm]{Pictures/5mdl_dual_H2_vU.jpg}
        %\caption{$3\sigma({}_{v}U)$}
        \caption{$\norm{u_v}_2$}
        \label{fig:dual:H2cst:vU}
    \end{subfigure}
    \begin{subfigure}[b]{8cm}
        \includegraphics[width=8cm]{Pictures/5mdl_dual_H2_mY_2.jpg}
        %\caption{$3\sigma({}_{m}Y)$}
        \caption{$\norm{y_m}_2$}
        \label{fig:dual:H2cst:mY}
    \end{subfigure}
    \caption{The $H_2$ norm constraints for the dual-stage loop over the iterations. The variances of signals is considered in the optimization problems, however the square roots of the variances, also known as the standard deviations, are plotted here. The triangles show the upper-bound of the standard deviations of the VCM control action (a) and the MA output stroke (b), where the circles show the real value of the standard deviations. The $H_2$ norm objective and constraints are activated starting from second and third iterations, respectively.}\label{fig:dual:H2cst}
\end{figure}

Fig.~\ref{fig:dual:H2obj} plots the standard deviation of the tracking error for the dual-stage feedback system in Fig.~\ref{fig:AppDD:DualSD}. According to Eqs. (\ref{eq:opt:sd:dual:II}) and (\ref{eq:opt:miso:II}), the minimization of square of this standard deviation, which is equal to the variance, is considered as the minimization objective in the SIMO design strategy as well as the second step of the sequential SISO design strategy. In the sequential SISO design strategy, the obtained VCM compensator $K_v$ may optimize the VCM single-stage $H_2$ norm objective by compromising the dual-stage $H_2$ norm objective, since the compensator $K_v$ design process in sequential SISO design strategy does not take into account the dual-stage loop. Fig.~\ref{fig:dual:H2obj} shows that the sequential SISO design strategy achieves relatively higher $H_2$ norm objective compared to the SIMO design strategy.

%The $H_2$ norm objective of minimizing the dual-stage tracking error has been plotted in Fig.~\ref{fig:dual:H2obj}. The $K_v$ designed in the SISO methodology does not take into account the dual-stage loop, therefore, the obtained $K_v$ controller may optimize the single-stage $H_2$ norm objective by compromising the dual-stage $H_2$ norm objective. Fig.~\ref{fig:dual:H2obj} shows that the SISO design methodology achieves relatively higher $H_2$ norm objective compared to the SIMO design methodology.

The results in Fig.~\ref{fig:dual:H2obj} also suggest that the standard deviation of the dual-stage tracking error in the MISO design strategy is a non-linear function of the restriction on the standard deviation of the MA output stroke. If the constraint on the MA output stroke given in Eq. (\ref{eq:dual:H2:mYnumbers}) is 42 nm or greater, the standard deviation of the dual-stage tracking error will not change significantly. The main reason is that the VCM in Fig.~\ref{fig:single:H2:S} will compensate for the MA output stroke restriction. However, the VCM ability to compensate for the MA output stroke restriction is limited. If the standard deviation upper-bound on the MA output stroke is smaller than 42 nm, the decrease in this upper-bound will increase the standard deviation of the dual-stage tracking error at a higher rate as compared to the case of the MA output stroke with the standard deviation of 42 nm or greater.


%If the standard deviation upper-bound on the MA output stroke becomes smaller than 42 nm, the standard deviation of the dual-stage tracking error will increase at a higher rate as compared to the case of the MA output stroke of larger than 42 nm.

%However, if the standard deviation upper-bound on the MA output stroke becomes smaller than 42 nm, the standard deviation of the dual-stage tracking error will increase at a higher rate, since the VCM ability to compensate for the MA output stroke restriction is limited.


%the VCM compensation for this restriction relatively reduces, and the standard deviation of the dual-stage tracking error will increase more.

%In terms of $H_2$ norm constraint on MA output, if this constraint has been restricted up to $0.7$, the dual-stage $H_2$ objective will not change significantly. The main reason is that the VCM in Fig. ... will compensate for this MA restriction. However, if the $H_2$ norm upper bound on the MA become smaller than $0.7$, the VCM cannot compensate for this restriction, and the $H_2$ objective of the dual-stage loop will increase.
\begin{figure}
	\centering
	\includegraphics[width=8cm]{Pictures/5mdl_dual_H2_S_2.jpg}
    \caption{$\norm{e}_2$: The $H_2$ norm objective for the dual-stage loop. The variances of signals is considered in the optimization problems, however the square roots of the variances, also known as the standard deviations, are plotted here. The $H_2$ norm objective and constraints are activated starting from second and third iterations, respectively.}
    \label{fig:dual:H2obj}
\end{figure}

% Dual: siso vs miso: bw & stability margin
% Dual: among miso
% Dual: Tr

%%% dual: Sr: siso vs miso
Table~\ref{table:dual:Margins} presents the dual-stage stability margins and bandwidths for the design scenarios considered in table~\ref{table:design:scenarios}. In this table, the open loop transfer function is from the track run-out r to the position head output y. The more restriction on the MA output stroke, which is achieved by reducing the upper-bound on the standard deviation of this signal, will compromise the dual-stage bandwidth. This reduction in the bandwidth will help to improve the stability margins. The dual-stage controller designed using the sequential SISO design strategy will have a relatively lower bandwidth and a higher peak for the sensitivity plot as compared to the $SIMO_4$ case. The higher sensitivity plot peak for the sequential SISO design strategy can be justified by the fact that this strategy will design compensators $k_v$ and $k_m$ in two individual steps and the compensator $K_v$ is designed without considering the dual-stage actuation structure.


%However, it can achieve higher stability margins compared to the SIMO methodology, because of its relatively low bandwidth. The lower bandwidth of the controller designed using SISO methodology can be justified, since the SISO methodology will design $k_v$ and $k_m$ in two individual steps and the $K_v$ has been designed without considering the dual-stage actuation structure.% by the peak around $2KHz$ in the dual-stage sensitivity plot in Fig.~\ref{fig:dual:Er}. This peak is a result of the aggressive VCM controller with relatively low stability margin. Moreover in the SISO methodology, the $K_v$ has been designed without considering the dual-stage actuation structure.
\begin{table}[ht]
\caption{Stability margins for the dual-stage loop} % title of Table
\centering % used for centering table
\begin{tabular}{c c c c c c} % centered columns (4 columns)
\hline\hline\\[-0.8em] %inserts double horizontal lines
Scenarios 				& 	$E_{r \rightarrow e}$ peak	&	$GM$ 	& $PM$ 		& 	$\omega_{GM}$ 	& 	$\omega_{PM}$\\ [0.5ex] 
		 			    &	$dB$		& 	$dB$ 	& $degree$ 	& 	$Hz$ 			& 	$Hz$ \\ [0.5ex]
\hline \\[-0.5em]
\text{$SIMO_1$}  &	9.63  & 8.85  &  19.13 	 & 	12,392 			& 	4,924    \\
\text{$SIMO_2$}  &	9.62  & 8.85  &  19.14 	 & 	12,393 			& 	4,922    \\
\text{$SIMO_3$}  &	9.55  & 8.86  &  19.36 	 &  12,390			& 	4,914    \\
\text{$SIMO_4$}  &	9.43  & 8.87  &  19.74	 &  12,401 			& 	4,884    \\
\text{$SISO_1$}  & 	9.58  & 8.90  &  19.23 	 & 	12,377 			&	4,857    \\ [1ex] % [1ex] adds vertical space
\hline %inserts single line
\end{tabular}
\label{table:dual:Margins} % is used to refer this table in the text
\end{table}

%%% dual: Sr: simo's
%As mentioned, increasing the restriction on the MA output in the SIMO design will result in more aggressive VCM controller to compensate for the additional restriction on MA output. However, since both $K_v$ and $K_m$ have been designed in one step with the objective of minimizing the $H_2$ norm of dual-stage tracking error, the increase in VCM bandwidth will help to increase the dual-stage bandwidth. In this case, increasing the dual-stage bandwidth will reduce the stability margin in terms of the sensitivity peak.

%%% dual: Tr
Fig.~\ref{fig:dual:Tr} plots the frequency response of the closed loop transfer functions from the track run-out r to the actuator outputs. As shown in the figure, the VCM actuator is more active at the low frequency region, while the MA actuator takes over at the mid-frequency region. At the high frequency region, the output of both actuators will reduce, since the system can not be controlled due to the dynamics uncertainty of the actuators.

Fig.~\ref{fig:SISO:noises} suggests that the magnitude of the run-out has an inverse relationship with the frequency. Therefore, the more restriction on the standard deviation of the MA output stroke defined in Eq. (\ref{eq:H2:mY:dual}) will force the MA output to be more active at higher frequency regions, where the magnitude of run-out is smaller. As shown in Fig.~\ref{fig:dual:Tr}, the controller with more restricted MA output stroke criteria will result in smaller MA output magnitude in frequencies between $500-2000~Hz$ and higher MA output magnitude in frequencies between $2000-3000~Hz$. According to Fig.~\ref{fig:dual:Er}, the smaller magnitude of the MA output in lower frequency regions sacrifices the tracking error rejection in those regions. At higher frequency regions, the larger magnitude of the MA output helps to improve the tracking error rejection.

%, which according to Fig.~\ref{fig:dual:Er} will sacrifice the tracking error rejection at those frequencies. However in frequencies around $2000-3000~Hz$, the higher magnitude of MA output will help to improve the tracking error rejection. %It is worth mentioning that the lower MA output activity in frequencies around $500-2000~Hz$ has also resulted in lower VCM activity, which is supporting the results in Table~\ref{fig:dual:H2cst}.

%reduce the MA output magnitude at lower frequencies and increase the MA output magnitude at higher frequencies. As one can see in Fig.~\ref{fig:dual:Tr}, the controller with more restricted MA output

%%% dual: Tr, peaks
%The $H_2$ norm constraints restrict the integration of the frequency response magnitude over the whole frequency region. Therefore, increasing the restriction on $H_2$ norm can lead to smaller $H_2$ norm but it can create sharp peaks at few frequency regions. As one can see in Fig.~\ref{fig:dual:H2cst:mY}, increasing the restriction on MA output, have reduced the $H_2$ norm of the MA output, but it has increased the magnitude of the pick in the frequency response plot of MA output in Fig.~\ref{fig:dual:Tr}. If the $H_2$ norm constraints create the peaks which reduce the stability margins or violate performance specifications, those peaks will be bounded by shaping the closed loop transfer functions using the weighted $H_\infty$ constraints.
\begin{figure}
    \centering
    \begin{subfigure}[b]{8cm}
        \includegraphics[width=8cm]{Pictures/5mdl_dual_Sr.jpg}
        \caption{$E_{r \rightarrow e}$}
        \label{fig:dual:Er}
    \end{subfigure}
    \begin{subfigure}[b]{8cm}
        \includegraphics[width=8cm]{Pictures/5mdl_dual_Tr_2.jpg}
        \caption{$Y_{r \rightarrow y_v, y_m}$}
        \label{fig:dual:Tr}
    \end{subfigure}
    \caption{The magnitude Bode plots of closed loop transfer functions for the dual-stage loop.}\label{fig:dual:SrTr}
\end{figure}



%%% controller order reduction
The frequency responses of the obtained compensators $K_v$ and $K_m$ are plotted in Fig.~\ref{fig:dual:K} for all the scenarios in table~\ref{table:design:scenarios}. The SIMO design strategy uses the stable factorizations of the controller in Eqs. (\ref{eq:MISO:fact:Xi}) and (\ref{eq:MISO:fact:Yi}) with the controller order parameter $n = 25$ in order to obtain the SIMO controller. After designing the SIMO controller, the compensators $K_v$ and $K_m$ are derived using Eqs. (\ref{eq:miso:KvKbar}) and (\ref{eq:miso:KmKbar}). The Hankel singular values~\cite{hankel2005} of these compensators are plotted in Fig.~\ref{fig:dual:KSigma}. In order to reduce the compensators orders, few of the Hankel singular values with the smallest magnitudes are eliminated. The gray boxes in Fig.~\ref{fig:dual:KSigma} show the eliminated Hankel singular values. The reduced order compensators $K_v$ and $K_m$ will be $17^{th}$ and $20^{th}$ orders, respectively. The comparisons between the reduced order and the full order compensators are also provided in Fig.~\ref{fig:dual:KSigma}. As one can notice, the compensator order reduction will not create any significant difference in low and mid frequency regions of the compensators frequency responses. In high frequency regions, the deviation between the reduced order and the full order VCM compensator $K_v$ will not significantly affect the closed loop transfer functions, since according to Fig.~\ref{fig:SISO:G}, the VCM response has relatively small magnitude at high frequency regions. Moreover, the effect of MA compensator order reduction at high frequency regions is negligible.




%The VCM controller order reduction in high frequency region will not significantly affect the closed loop transfer functions , since according to Fig.~\ref{fig:SISO:G}, VCM has relatively small response at high frequency regions. Moreover, the effect of MA controller order reduction at high frequency region is negligible.  %it is damped by relatively sm, the deviation is less than $2dB$.
\begin{figure}
	\centering
	\includegraphics[width=8cm]{Pictures/5mdl_dual_K.jpg}
    \caption{The compensators $K_v$ and $K_m$ for the design scenarios in table~\ref{table:design:scenarios}. The compensator $K_v$ is denoted with thick lines, where the compensator $K_m$ is denoted with thin lines.}
    \label{fig:dual:K}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}[b]{8cm}
        \includegraphics[width=8cm]{Pictures/5mdl_dual_KvSigma_2.jpg}
        \caption{$K_v$}
        \label{fig:dual:KvSigma}
    \end{subfigure}
    \begin{subfigure}[b]{8cm}
        \includegraphics[width=8cm]{Pictures/5mdl_dual_KmSigma_2.jpg}
        \caption{$K_m$}
        \label{fig:dual:KmSigma}
    \end{subfigure}
    \caption{The Hankel singular values for both $K_v$ and $K_m$ compensators. The gray boxes show the singular values which are eliminated for the purpose of compensator order reduction.}\label{fig:dual:KSigma}
\end{figure}

%As mentioned, the controllers $K_v$ and $K_m$ for the SISO design methodology are designed in two individual steps. In the second step, the optimization problem (..) is solving for the $K_m$ without having any flexibility to change the designed $K_m$. As it was shown in Fig.~\ref{fig:dual:H2obj} and Table~\ref{table:dual:Margins}, this restriction can sacrifice the dual-stage performance in terms of $H_2$ objective as well as reducing the bandwidth of the dual-stage loop.

%As mentioned earlier, the SISO design methodology first solves for the controller $K_v$ considering the single-stage loop. Then, the controller $K_m$ is solved for the dual-stage loop without having any flexibility to change the designed $K_v$ in the previous step. As it was shown in Fig.~\ref{fig:dual:H2obj} and Table~\ref{table:dual:Margins}, this restriction can sacrifice the dual-stage performance in terms of $H_2$ objective as well as reducing the bandwidth of the dual-stage loop. However, this restriction may cause the convex optimization problem in Eq. (..) to be infeasible, in the case that the MISO methodlogy can find a feasible solution to the equivalent optimization problem in Eq. (..).

\subsubsection{A limitation of Sequential SISO Design Strategy}
It is worth mentioning that if the SIMO design strategy is successful to find a feasible solution for the optimization problem in Eq. (\ref{eq:opt:miso:II}), there is no guarantee that the sequential SISO design strategy can also find a feasible solution for the optimization problem in Eq. (\ref{eq:opt:sd:dual:II}). As an example, the weighting function used in the $H_\infty$ norm of the closed loop transfer function $U_{w_v \rightarrow u_m}$ in the above example is adjusted to force more restriction at high frequency regions. In Fig.~\ref{fig:dual:inf}, the previous $H_\infty$ constraint limit is shown with light blue dotted lines, while the new $H_\infty$ constraint limit is shown with red dotted lines. The MISO design strategy is able to find a controller which can satisfy the new constraint. However, the sequential SISO design strategy is not able to find a feasible solution to satisfy this new constraint, since this strategy designs the compensator $K_v$ without considering the dual-stage loop constraints, and also the compensator $K_m$ is designed for the dual-stage loop without having the flexibility to change the compensator $K_v$.

\begin{figure}
	\centering
	\includegraphics[width=8cm]{Pictures/5mdl_dual_infeasible.jpg}
    \caption{The magnitude Bode plots of the closed loop transfer function from control input disturbance $w_v$ to MA control input $u_m$, $U_{w_v \rightarrow u_m}$. The red dotted lines represent the restricted $H_\infty$ constraint limit, while the light blue dotted lines represent the $H_\infty$ constraint limit used in this section. The SIMO design strategy obtains the controller such that $U_{w_v \rightarrow u_m}$ transfer functions satisfy the restricted $H_\infty$ constraint limit. The sequential SISO design strategy cannot find a feasible solution for this restricted $H_\infty$ constraint limit.}
    \label{fig:dual:inf}
\end{figure}


\subsubsection{Comparison Between $H_\infty$ Conditions in Section~\ref{sec:DD:ControlAlgorithm}}
%%%%%%%%%%%%
% LMI vs. Ineq.
%%%%%%%%%%%%
The results presented in this section, use theorem~\ref{THEOREMMISOHINF} to find necessary and sufficient convex conditions for the $H_\infty$ constraints considered in the optimization problems given in Eqs. (\ref{eq:opt:sd:single:II})-(\ref{eq:opt:miso:II}). As mentioned in section~\ref{sec:DD:ControlAlgorithm}, sufficient convex conditions for the $H_\infty$ constraints has been proposed in~\cite{karimi2016H2}. These two types of convex conditions for the $H_\infty$ constraints can be summarized as

\begin{itemize}
\item  I) necessary and sufficient convex conditions given in theorem~\ref{THEOREMMISOHINF},% in the mixed $H_2/H_\infty$ criteria.
\item  II) sufficient convex conditions given in theorem~\ref{theorem:miso:Hinf:Karimi}.% in the mixed $H_2/H_\infty$ criteria.
\end{itemize}

In order to compare these two convex conditions for the $H_\infty$ constraints, the dual-stage controller in Fig.~\ref{fig:AppDD:DualSD} is obtained by solving the mixed $H_2/H_\infty$ control design problem given in Eq.~(\ref{eq:opt:miso:II}). All the designed controllers satisfy the $H_\infty$ and $H_2$ norm constraints. The $H_2$ norm objectives for these two conditions are compared in Fig.~\ref{fig:HDDAPP:LMIvsIneq}, where the circle ($\circ$) and cross ($\times$) marks respectively represent conditions I and II as the convex conditions for the $H_\infty$ constraints. As one can notice, the sufficient $H_\infty$ conditions denoted as condition II will compromise the minimization objective as compared to the necessary and sufficient $H_\infty$ conditions denoted as condition I for all the MISO design scenarios introduced in table~\ref{table:design:scenarios}. The degraded performance for condition II can be justified by the fact that having only sufficient conditions for the $H_\infty$ constraints introduces conservatism in the optimization problem and leads to an increase in the minimization objective as compared to the necessary and sufficient conditions.% and degrad

%is able to achieve smaller minimization objective. the minimization objective which is the norm two of the dual-stage tracking error

\begin{figure}
	\centering
	\includegraphics[width=8cm]{Pictures/LMIvsIneq_2.jpg}
    \caption{The $H_2$ norm objective for the dual-stage loop. The variances of signals is considered in the optimization problems, however the square roots of the variances, also known as the standard deviations, are plotted here. The circle ($\circ$) and cross ($\times$) marks respectively represent conditions I and II as the convex conditions for the $H_\infty$ constraints used in Eq.~(\ref{eq:opt:miso:II}). The $H_2$ norm objective and constraints are considered in the optimization problem starting from the second and third iterations, respectively.}
    \label{fig:HDDAPP:LMIvsIneq}
\end{figure}

